A Real-Time, GPU-Based, Non-Imaging Back-End for Radio Telescopes

Since the discovery of RRATs, interest in single pulse radio searches has increased dramatically. Due to the large data volumes generated by these searches, especially in planned surveys for future radio telescopes, such searches have to be conducted in real-time. This has led to the development of a multitude of search techniques and real-time pipeline prototypes. In this work we investigated the applicability of GPUs. We have designed and implemented a scalable, flexibile, GPU-based, transient search pipeline composed of several processing stages, including RFI mitigation, dedispersion, event detection and classification, as well as data quantisation and persistence. These stages are encapsulated as a standalone framework. The optimised GPU implementation of direct dedispersion achieves a speedup of more than an order of magnitude when compared to an optimised CPU implementation. We use a density-based clustering algorithm, coupled with a candidate selection mechanism to group detections caused by the same event together and automatically classify them as either RFI or of celestial origin. This setup was deployed at the Medicina BEST-II array where several test observations were conducted. Finally, we calculate the number of GPUs required to process all the beams for the SKA1-mid non-imaging pipeline. We have also investigated the applicability of GPUs for beamforming, where our implementation achieves more than 50% of the peak theoretical performance. We also demonstrate that for large arrays, and in observations where the generated beams need to be processed outside of the GPU, the system will become PCIe bandwidth limited. This can be alleviated by processing the synthesised beams on the GPU itself, and we demonstrate this by integrating the beamformer to the transient detection pipeline.

==> abstract.tex <==
\onehalfspacing

Since the discovery of Rapidly Rotating Transients (RRATs), interest in single pulse radio searches has increased dramatically.  Due to the large data volumes generated by these searches, especially in planned surveys for future radio telescopes, such searches have to be conducted in real-time. This has led to the development of a multitude of search techniques and real-time pipeline prototypes. In this work we investigated the applicability of GPUs for such systems. 

We have designed and implemented a scalable, flexibile, GPU-based, transient search pipeline composed of several processing stages, including RFI mitigation, dedispersion, event detection and classification, as well as data quantisation and persistence. These stages are encapsulated as a standalone framework which can be used in offline mode, for processing archival data, as well as within an online application with additional real-time capabilities. The optimised GPU implementation of direct dedispersion achieves a speedup of more than an order of magnitude when compared to an optimised CPU implementation. We use a density-based clustering algorithm, coupled with a candidate selection mechanism to group detections caused by the same event together and automatically classify them as either RFI or of celestial origin. This setup was deployed at the Medicina BEST-II array in Italy, attached to an FPGA-based digital backend where several test observations were conducted. Finally, we calculate the number of GPUs required to process all the beams for the SKA$_1$-mid non-imaging pipeline.

We have also investigated the applicability of GPUs for beamforming, where our implementation achieves more than 50\% of the peak theoretical performance. We also demonstrate that for large arrays, and in observations where the generated beams need to be processed outside of the GPU, the system will become PCIe bandwidth limited, with the attached GPUs spending most of the execution time waiting for I/O transfers. This can be alleviated by processing the synthesised beams on the GPU itself, and we demonstrate this by integrating the beamformer to the transient detection pipeline. We also analysed the beamforming computational requirements for SKA$_1$-low and SKA$_1$-mid, and demonstrate that GPUs are an inefficient architecture for this, with a very high running cost.


==> ack.tex <==
\onehalfspacing

I'm not really sure how I ended up doing a PhD, but I'm pretty certain that my supervisor, Dr Kristian Zarb Adami, had something to do with it. I have no regrets, it's been an interesting and rewarding journey. Thanks for everything, you deserves endless hugging. A big thanks also goes to my co-supervisor, Dr. John Abela, who thinks that someday he'll manage to eat more than I can.

Thanks to Aris Karastergiou for answering endless streams of questions about everything transient, and for setting in motion all the processes which would culminate in me writing this thesis. A big thanks to the dynamic SKA group at the University of Oxford and Oxford e-Research Centre, with people deserving special mention including: Ian Heywood, Sascha Schediwy, Stef Salvini, Fred Dulwich, Benjamin Mort, Wes Armour and especially Steve Rawlings, who will always be remembered in the hearts and minds of everyone who knew him. A big thanks goes to the ``digital team'', namely Jack Hickish, Griffin Foster, Richard Armstrong and Danny Price, for making every trip to Oxford one to remember, and their immeasurable patience in dealing with my nagging.

I also thank the staff and support from Radiotelescopi di Medicina whom made the deployment at the BEST-II array possible, particularly Andrea Mattana, Frederico Perini, Germano Bianchi,
Giovanni Naldi, Jader Monari, Marco Bartolini, and Stelio Montebugnoli. Thanks also go to Andrew Siemion, Mark Wagner, Dan Werthimer and other people at CASPER, Berkeley, USA.

It's been a blast working at the department of physics in the University of Malta. Special thanks goes to Prof. Charles Sammut, our beloved dean, the lovely Alison Darmanin and the rest of the department and faculty staff. Thanks to the founding member of the AstroMalta team: Jackson Said, Ian Fenech Conti, Adam Gauci, as well as the crazy students in the APRR. It's been awesome!

I'd also like to thank in advance my examiners, Dr. Scott Ransom and Dr. Rob Fender. Last, but surely not least, I'd like to thank my family and friends for their endless and unquestioning support. I'm sure I forgot to mention a great number of people, but worry not, I thank you!




==> acronyms.tex <==

{\setlength{\extrarowheight}{10pt}

\begin{table}[ht!]
 \begin{tabular} {  p{2.2cm}  p{11.5cm} }
  ADC      & Analog to Digital Converter \\
  ARTEMIS  & Advanced Radio Transients Event Monitor and Identification System \\
  ASM      & All Sky Monitor \\
  AVX      & Advanced Vector Extensions \\
  BEST     & Basic Element for SKA Training  \\
  CASPER   & Collaboration for Astronomy Signal Processing and Electronics Research \\
  CMAC     & Complex Multiply-Accumulate \\
  CPU      & Central Processing Unit \\
  CRAFT    & Commensal Real-time ASKAP Fast Transients \\
  CSP      & Central Signal Processing \\
  CUDA     & Compute Unified Device Architecture \\
  DDR      & Double Data Rate \\
  DBSCAN   & Density-Based Spatial Clustering of Applications with Noise  \\
  DM       & Dispersion Measure  \\
  FFT      & Fast Fourier Transform \\
  FLOP     & Floating Point Operation \\
  FoV      & Field of View \\
  FoMSS    & Figure of Merit Survey Speed \\
  FPGA     & Field Programmable Gate Array \\
  FRB      & Fast Radio Bursts \\
  \end{tabular}
\end{table}


\begin{table}[t!]
 \begin{tabular} { p{2.2cm}  p{11.5cm} }
  FWHM     & Full Width Half Maximum \\
  GbE      & Gigabit Ethernet \\
  GPU      & Graphics Processing Unit\\
   ILP      & Instruction Level Parallelism  \\ 
  LOFAR    & Low Frequency Array \\
  PCI      & Peripheral Component Interconnect \\
  PFB      & Polyphase Filter Bank \\
  RFI      & Radio Frequency Interference \\
  RAM      & Random Access Memory \\
  RMSE     & Root Mean Square Error \\
  ROACH    & Reconfigurable Open Architecture Computing Hardware \\ 
  RRAT     & Rapidly Rotating Transient \\
  SKA      & Square Kilometer Array \\
  S/N      & Signal-to-Noise \\
  SPEAD    & Streaming Protocol for Exchanging Astronomical Data \\
  TDP      & Thermal Design Power \\
  UDP      & User Datagram Protocol \\
  XAUI     & Ten Gigabit Attachment Unit Interface
 \end{tabular}
\end{table}
}

{\tiny .}

==> publications.tex <==
\section*{Refereed Publications}

\begin{itemize}
 \item {\bf Magro A.}, Karastergiou A., Salvini S., Mort B., Dulwich F. and Zarb Adami, K. (2011). Real-time, fast radio transient searches with GPU de-dispersion. Monthly Notices of the Royal Astronomical Society, 17, 2642-2650.

 \item {\bf Magro A.}, Hickish J. and Zarb Adami K.(2013). Mulitbeam GPU Transient Pipeline for the Medicina BEST-2 Array. Journal of Astronomical Instrumentation. 2 (1).
 
 \item Foster G., Hickish J., {\bf Magro A.}, Price D. and Zarb Adami K. (2013). Implementation of a Direct-Imaging and FX Correlator for
the BEST-2 Array. Accepted for publication in Monthly Notices of the Royal Astronomical Society

 
\end{itemize}


\section*{Conference Contributions}

\begin{itemize}
 \item  Armour W., Karastergiou A., Giles M., Williams C., {\bf Magro A.}, Zagkouris K., Roberts S., Salvini S., Dulwich F. and Mort B. (2012). A GPU-based survey for millisecond radio transients using ARTEMIS. In ASP
Conference Series p. 33.
\item {\bf Magro A.} and Zarb Adami K. (2013). Pipeline Prototype for Fast Radio Transient Detection Using GPUs. 5$^{\text{th}}$ Workshop in Information and Communications Technology. SmartCity Malta

\item Zheng H., Tegmark M. {\it et al}. (2013). Mapping our Universe in 3D with MITEoR. To be published in proceedings of 2013 IEEE International Symposium on Phased Array Systems and Technology

\end{itemize}

\section*{In Preparation}
\begin{itemize}
 
\item Zarb Adami K. and {\bf Magro A.}. (2013).  GPU-Based Beamforming for Transient Discovery. {\it In prep.}

\end{itemize}


